Leasing the Cloud-Edge Continuum, \`a la Carte

Next-gen computing paradigms foresee deploying applications to virtualised resources along a continuum of Cloud-Edge nodes. Much literature focussed on how to place applications onto such resources so as to meet their requirements. To lease resources to application operators, infrastructure providers need to identify a portion of their Cloud-Edge assets to meet set requirements. This article proposes a novel declarative resource selection strategy prototyped in Prolog to determine a suitable infrastructure portion that satisfies all requirements. The proposal is showcased over a lifelike scenario.

==> eptcsdata.tex <==
\providecommand{\firstpage}{288}
\providecommand{\publicationstatus}{S. Costantini, E. Pontelli, A. Russo, F. Toni,\\R. Calegari, A. D'Avila Garcez, C. Dodaro, F. Fabiano,\\ S. Gaggl, A. Mileo, (Eds.): ICLP 2023\\
EPTCS 385, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.385.28}{10.4204/EPTCS.385.28}}
\pdfoutput=1

